Impostor Syndrome in Final Year Computer Science Students: An Eye Tracking and Biometrics Study

Imposter syndrome is a psychological phenomenon that affects individuals who doubt their skills and abilities, despite possessing the necessary competencies. This can lead to a lack of confidence and poor performance. While research has explored the impacts of imposter syndrome on students and professionals in various fields, there is limited knowledge on how it affects code comprehension in software engineering. In this exploratory study, we investigate the prevalence of imposter syndrome among final-year undergraduate computer science students and its effects on their code comprehension cognition using an eye tracker and heart rate monitor. Key findings demonstrate that students identifying as male exhibit lower imposter syndrome levels when analyzing code, and higher imposter syndrome is associated with increased time reviewing a code snippet and a lower likelihood of solving it correctly. This study provides initial data on this topic and establishes a foundation for further research to support student academic success and improve developer productivity and mental well-being.

==> table_all_aoi_type.tex <==
\begin{table}[]
\vspace{-15pt}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{llllllllllll}
 &
  variable decl &
  else stmt &
  for loop &
  if stmt &
  import stmt &
  method call &
  method decl &
  recursive method call &
  return stmt &
  variable asgmt &
  Multiple \\
Few IPC      & 10   & \cellcolor[HTML]{32CB00}4.5 & 7.8                         & 8.2 & 10.6 & 10.9 & \cellcolor[HTML]{FD6864}17.7 & 8.6  & 11.3 & 9.6 & 1 \\
Moderate IPC &
  8.2 &
  8.2 &
  7 &
  7.9 &
  9.2 &
  7.5 &
  9.3 &
  \cellcolor[HTML]{FD6864}24.8 &
  \cellcolor[HTML]{32CB00}{\color[HTML]{333333} 6.1} &
  9.4 &
  2.5 \\
Frequent IPC & 10.4 & 6.9                         & \cellcolor[HTML]{32CB00}6.5 & 7.2 & 11.6 & 12   & \cellcolor[HTML]{FD6864}15.5 & 11.7 & 8.9  & 8.2 & 1 \\
Intense IPC &
  7.8 &
  10.6 &
  6.6 &
  \cellcolor[HTML]{32CB00}5.3 &
  8.9 &
  12.4 &
  \cellcolor[HTML]{FD6864}{\color[HTML]{333333} 17.4} &
  16.1 &
  6.3 &
  6.1 &
  2.5
\end{tabular}%
}
\vspace{-15pt}
\end{table}

==> table_clanceIP_range.tex <==
\begin{table}[]
\vspace{-15pt}
\caption{Range of values associated with each IPC level}
\label{Table:clanceIPRange}
\begin{tabular}{ll}
\hline
\textbf{IPC Level} & \textbf{Scores} \\ \hline
Few                & \textless  40   \\ \hline
Moderate           & 41 - 60         \\ \hline
Frequent           & 61 - 80         \\ \hline
Intense            & \textgreater 80 \\ \hline
\end{tabular}
\vspace{-15pt}
\end{table}

==> table_correlations_grand.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[H]
\vspace{-15pt}
\caption{Correlation Matrix of Averages across Snippets}
\label{Table:corr_matrix_biometrics}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{rrrrrrrr}
\multicolumn{1}{l}{} &
  \multicolumn{1}{c}{\textit{\textbf{M}}} &
  \multicolumn{1}{c}{\textit{\textbf{SD}}} &
  \multicolumn{1}{c}{\textit{\textbf{\begin{tabular}[c]{@{}c@{}}IP \\ Score\end{tabular}}}} &
  \multicolumn{1}{c}{\textit{\textbf{\begin{tabular}[c]{@{}c@{}}Average \\ Heart Rate\end{tabular}}}} &
  \multicolumn{1}{c}{\textit{\textbf{\begin{tabular}[c]{@{}c@{}}Time \\ Spent\end{tabular}}}} &
  \multicolumn{1}{c}{\textit{\textbf{\begin{tabular}[c]{@{}c@{}}Correctly \\ Answered\end{tabular}}}} &
  \multicolumn{1}{c}{\textit{\textbf{Confidence}}} \\ \hline
\textbf{IP Score}           & 58.73  & 15.74 & \multicolumn{1}{c}{-} &                       &                       &                       &                       \\
\textbf{Average Heart Rate} & 84.39  & 9.29  & 0.04                  & \multicolumn{1}{c}{-} &                       &                       &                       \\
\textbf{Time Spent}         & 112.26 & 46.13 & 0.52*                 & 0.18                  & \multicolumn{1}{c}{-} &                       &                       \\
\textbf{Correctly Answered} & 0.29   & 0.23  & -0.52*                & -0.08                 & -0.34                 & \multicolumn{1}{c}{-} &                       \\
\textbf{Confidence}         & 3.53   & 0.65  & -0.37                 & 0.26                  & -0.49                 & 0.49                  & \multicolumn{1}{c}{-} \\ \hline
\end{tabular}%
}
\textbf{Notes: }* Correlation is significant at the 0.05 level
\vspace{-15pt}
\end{table}

==> table_correlations_grand_aoi.tex <==
\begin{table}[]
\vspace{-15pt}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{rrrcl}
\multicolumn{1}{l}{} &
  M &
  SD &
  \multicolumn{1}{l}{IPC Score} &
   \\ \hline
\multirow{2}{*}{\textbf{else-statement}} &
  \multirow{2}{*}{1.47} &
  \multirow{2}{*}{1.51} &
  0.46 &
  Pearson Correlation \\
 &
   &
   &
  0.08 &
  Sig. (2-tailed) \\
\multirow{2}{*}{\textbf{for-loop}} &
  \multirow{2}{*}{0.97} &
  \multirow{2}{*}{0.6} &
  0.4 &
  Pearson Correlation \\
 &
   &
   &
  0.14 &
  Sig. (2-tailed) \\
\multirow{2}{*}{\textbf{if-statement}} &
  \multirow{2}{*}{1.08} &
  \multirow{2}{*}{0.74} &
  0.2 &
  Pearson Correlation \\
 &
   &
   &
  0.47 &
  Sig. (2-tailed) \\
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}r@{}}import\\ statement\end{tabular}}} &
  \multirow{2}{*}{1.15} &
  \multirow{2}{*}{1.43} &
  0.35 &
  Pearson Correlation \\
 &
   &
   &
  0.2 &
  Sig. (2-tailed) \\
\multirow{2}{*}{\textbf{method call}} &
  \multirow{2}{*}{1.15} &
  \multirow{2}{*}{0.7} &
  0.56* &
  Pearson Correlation \\
 &
   &
   &
  0.03 &
  Sig. (2-tailed) \\
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}r@{}}method \\ declaration\end{tabular}}} &
  \multirow{2}{*}{1.87} &
  \multirow{2}{*}{0.99} &
  0.52* &
  Pearson Correlation \\
 &
   &
   &
  0.05 &
  Sig. (2-tailed) \\
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}r@{}}recursive \\ method call\end{tabular}}} & \multirow{2}{*}{2.09} & \multirow{2}{*}{1.7} & 0.27 & Pearson Correlation \\
 &
   &
   &
  0.33 &
  Sig. (2-tailed) \\
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}r@{}}return\\ statement\end{tabular}}} &
  \multirow{2}{*}{1.17} &
  \multirow{2}{*}{0.73} &
  0.1 &
  Pearson Correlation \\
 &
   &
   &
  0.72 &
  Sig. (2-tailed) \\
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}r@{}}variable\\ assignment\end{tabular}}} &
  \multirow{2}{*}{1.35} &
  \multirow{2}{*}{1.04} &
  0.13 &
  Pearson Correlation \\
 &
   &
   &
  0.64 &
  Sig. (2-tailed) \\
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}r@{}}variable\\ declaration\end{tabular}}} &
  \multirow{2}{*}{1.25} &
  \multirow{2}{*}{0.64} &
  0.36 &
  Pearson Correlation \\
 &
   &
   &
  0.19 &
  Sig. (2-tailed) \\
\multirow{2}{*}{\textbf{multiple}} &
  \multirow{2}{*}{0.31} &
  \multirow{2}{*}{0.35} &
  0.13 &
  Pearson Correlation \\
 &
   &
   &
  0.66 &
  Sig. (2-tailed) \\ \hline
\end{tabular}%
}
\vspace{-15pt}
\end{table}

==> table_ttest_ipc_gender.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}
\vspace{-15pt}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|c|c|c|c|cr|rlr|cr|}
\cline{2-4} \cline{6-7} \cline{11-12}
 &
  \multirow{2}{*}{\textit{F}} &
  \multirow{2}{*}{\textit{Sig.}} &
  \multirow{2}{*}{\textit{t}} &
   &
  \multicolumn{2}{c|}{Significance} &
  \multicolumn{1}{l}{} &
   &
  \multicolumn{1}{l|}{} &
  \multicolumn{2}{c|}{95\% CI} \\ \cline{5-12} 
 &
   &
   &
   &
  \textit{df} &
  \multicolumn{1}{c|}{\textit{One-Sided p}} &
  \multicolumn{1}{c|}{\textit{Two-Sided p}} &
  \multicolumn{2}{c|}{\textit{Mean Difference}} &
  \multicolumn{1}{c|}{\textit{Std. Error Difference}} &
  \multicolumn{1}{c|}{\textit{Lower}} &
  \multicolumn{1}{c|}{\textit{Upper}} \\ \hline
\multicolumn{1}{|r|}{\textbf{Equal variances assumed}} &
  \multicolumn{1}{r|}{.016} &
  \multicolumn{1}{r|}{.901} &
  \multicolumn{1}{r|}{-2.658} &
  \multicolumn{1}{r|}{12} &
  \multicolumn{1}{r|}{.010} &
  .021 &
  \multicolumn{2}{r|}{-18.244} &
  6.864 &
  \multicolumn{1}{r|}{-33.199} &
  -3.290 \\ \hline
\multicolumn{1}{|r|}{\textbf{Equal variances not assumed}} &
  \multicolumn{1}{r|}{} &
  \multicolumn{1}{r|}{} &
  \multicolumn{1}{r|}{-2.661} &
  \multicolumn{1}{r|}{8.412} &
  \multicolumn{1}{r|}{.014} &
  .028 &
  \multicolumn{2}{r|}{-18.244} &
  6.856 &
  \multicolumn{1}{r|}{-33.921} &
  -2.568 \\ \hline
\end{tabular}%
}
\vspace{-15pt}
\end{table}
